Contrastive Self-Supervised Learning for Skeleton Representations

Human skeleton point clouds are commonly used to automatically classify and predict the behaviour of others. In this paper, we use a contrastive self-supervised learning method, SimCLR, to learn representations that capture the semantics of skeleton point clouds. This work focuses on systematically evaluating the effects that different algorithmic decisions (including augmentations, dataset partitioning and backbone architecture) have on the learned skeleton representations. To pre-train the representations, we normalise six existing datasets to obtain more than 40 million skeleton frames. We evaluate the quality of the learned representations with three downstream tasks: skeleton reconstruction, motion prediction, and activity classification. Our results demonstrate the importance of 1) combining spatial and temporal augmentations, 2) including additional datasets for encoder training, and 3) and using a graph neural network as an encoder.

==> Skeleton Embeddings – NeurIPS SSL Workshop 2022/tables/ablations_color.tex <==
\newcommand{\separator}[1]{\midrule \multicolumn{6}{c}{\textsc{#1}}\\\midrule}

\begin{table}[t]
\centering
\caption{Effect of various ablations for training skeleton representations with SimCLR on downstream tasks. Each cell denotes mean performance and standard deviation across 3 different random seeds. For each row in the table, we pre-train 3 different encoder networks/linear classifiers using SimCLR and train each network on the downstream task with a frozen backbone. Baseline configuration has all augmentations (except random rotation), is trained with the full training set size, and was pre-trained with all five skeleton datasets. We highlighted changes over 8\% in bold.}
\label{table:ablations}
\begin{scriptsize}
\hspace*{-1.3cm}
\begin{tabular}{
    >{\raggedleft\arraybackslash}m{2.5cm}%
    >{\centering\arraybackslash}m{2.2cm}%
    @{\hspace{0.5cm}}%
    >{\centering\arraybackslash}m{2.2cm}%
    @{\hspace{0.5cm}}%
    >{\centering\arraybackslash}m{2.2cm}%
    @{\hspace{0.5cm}}%
    >{\centering\arraybackslash}m{2.2cm}%
    @{\hspace{0.5cm}}%
    >{\centering\arraybackslash}m{2.2cm}%
}
\toprule

& \multicolumn{2}{c}{\textbf{\textsc{Skeleton Reconstruction}}} & \multicolumn{2}{c}{\textbf{\textsc{Motion Prediction}}} & \textbf{\textsc{Activity Class.}} \\[0.1cm]
& \multicolumn{2}{c}{\textsc{Mean Absolute Error} (mm)} & \multicolumn{2}{c}{\textsc{Mean Absolute Error} (mm)} & \textsc{Accuracy} (\%) \\
& \multicolumn{2}{c}{\textit{Lower is better}} & \multicolumn{2}{c}{\textit{Lower is better}} & \textit{Higher is better} \\[0.1cm]
& \textsc{NTU-60} & \textsc{HDM05} & \textsc{NTU-60} & \textsc{HDM05} & \textsc{NTU-60}  \\

\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textsc{Baseline} & %
    \cellcolor[rgb]{0.9657, 0.9672, 0.9681} 62.0 ($\pm$ 2.3) &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 49.7 ($\pm$ 1.5) &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 52.1 ($\pm$ 0.6) &  % NTU motion prediction
    \cellcolor[rgb]{0.9657, 0.9672, 0.9681} 23.4 ($\pm$ 1.0) &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 45.8 ($\pm$ 1.0) \\ % NTU activity classification

\textsc{Finetuning} & %
    \cellcolor[rgb]{0.8780, 0.9257, 0.9519} 65.7 ($\pm$ 1.7), $\Delta$+3.7 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.8002, 0.8882, 0.9356} 55.0 ($\pm$ 2.9), \textbf{$\Delta$+5.3} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.8430, 0.9091, 0.9455} 56.5 ($\pm$ 1.2), \textbf{$\Delta$+4.4} &  % NTU motion prediction
    \cellcolor[rgb]{0.0196, 0.1882, 0.3804}\color{white} 44.7 ($\pm$ 3.2), \textbf{$\Delta$+21.3} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.6577, 0.0812, 0.1622}\color{white} 64.7 ($\pm$ 1.0), \textbf{$\Delta$+18.9} \\ % NTU activity classification

\textsc{30 FPS} & %
    \cellcolor[rgb]{0.9728, 0.9493, 0.9354} 60.8 ($\pm$ 0.7), $\Delta$-1.2 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.8430, 0.9091, 0.9455} 53.8 ($\pm$ 1.6), \textbf{$\Delta$+4.1} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 52.8 ($\pm$ 0.6), $\Delta$+0.7 &  % NTU motion prediction
    \cellcolor[rgb]{0.0196, 0.1882, 0.3804}\color{white} 37.1 ($\pm$ 0.6), \textbf{$\Delta$+13.7} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 45.1 ($\pm$ 0.1), $\Delta$-0.7 \\ % NTU activity classification

\textsc{MLP Backbone} & %
    \cellcolor[rgb]{0.9073, 0.9396, 0.9573} 64.6 ($\pm$ 2.3), $\Delta$+2.6 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.6161, 0.7947, 0.8830} 58.8 ($\pm$ 3.3), \textbf{$\Delta$+9.1} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.7421, 0.8587, 0.9190} 59.0 ($\pm$ 2.3), \textbf{$\Delta$+6.9} &  % NTU motion prediction
    \cellcolor[rgb]{0.3599, 0.6380, 0.7979}\color{white} 29.7 ($\pm$ 1.5), \textbf{$\Delta$+6.3} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.1791, 0.4657, 0.7081}\color{white} 29.3 ($\pm$ 0.9), \textbf{$\Delta$-16.5} \\ % NTU activity classification



\separator{Downstream Task Training Set Size}
\textsc{15\%} & %
    \cellcolor[rgb]{0.9783, 0.9234, 0.8911} 59.5 ($\pm$ 0.9), $\Delta$-2.5 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9014, 0.9368, 0.9562} 52.0 ($\pm$ 0.8), $\Delta$+2.3 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.7712, 0.8734, 0.9273} 58.3 ($\pm$ 1.0), \textbf{$\Delta$+6.2} &  % NTU motion prediction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 23.7 ($\pm$ 0.9), $\Delta$+0.3 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.7033, 0.8390, 0.9080} 39.1 ($\pm$ 1.7), \textbf{$\Delta$-6.7} \\ % NTU activity classification

\textsc{10\%} & %
    \cellcolor[rgb]{0.9829, 0.9019, 0.8542} 58.2 ($\pm$ 0.6), $\Delta$-3.8 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.8839, 0.9285, 0.9530} 52.6 ($\pm$ 1.2), $\Delta$+2.9 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.7227, 0.8488, 0.9135} 59.4 ($\pm$ 0.7), \textbf{$\Delta$+7.3} &  % NTU motion prediction
    \cellcolor[rgb]{0.0196, 0.1882, 0.3804}\color{white} 54.3 ($\pm$ 2.3), \textbf{$\Delta$+30.9} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.5968, 0.7849, 0.8775} 37.1 ($\pm$ 1.0), \textbf{$\Delta$-8.7} \\ % NTU activity classification

\textsc{5\%} & %
    \cellcolor[rgb]{0.9839, 0.8976, 0.8468} 57.9 ($\pm$ 0.5), $\Delta$-4.1 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.0498, 0.2464, 0.4611}\color{white} 73.1 ($\pm$ 1.3), \textbf{$\Delta$+23.4} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.0498, 0.2464, 0.4611}\color{white} 76.7 ($\pm$ 4.0), \textbf{$\Delta$+24.6} &  % NTU motion prediction
    \cellcolor[rgb]{0.0196, 0.1882, 0.3804}\color{white} 73.5 ($\pm$ 6.6), \textbf{$\Delta$+50.1} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.3478, 0.6303, 0.7938}\color{white} 33.3 ($\pm$ 0.4), \textbf{$\Delta$-12.5} \\ % NTU activity classification



\separator{SimCLR Pre-training datasets}
\textsc{w/o Trinity} & %
    \cellcolor[rgb]{0.9746, 0.9406, 0.9206} 60.4 ($\pm$ 0.4), $\Delta$-1.6 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 49.6 ($\pm$ 0.9), $\Delta$-0.1 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 51.9 ($\pm$ 0.6), $\Delta$-0.2 &  % NTU motion prediction
    \cellcolor[rgb]{0.9540, 0.9617, 0.9659} 23.6 ($\pm$ 0.8), $\Delta$+0.2 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9248, 0.9479, 0.9606} 44.5 ($\pm$ 1.5), $\Delta$-1.3 \\ % NTU activity classification

\textsc{w/o TWH} & %
    \cellcolor[rgb]{0.9765, 0.9320, 0.9059} 60.0 ($\pm$ 0.2), $\Delta$-2.0 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 50.3 ($\pm$ 0.7), $\Delta$+0.6 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9599, 0.9645, 0.9670} 52.4 ($\pm$ 0.4), $\Delta$+0.3 &  % NTU motion prediction
    \cellcolor[rgb]{0.9700, 0.9622, 0.9576} 23.3 ($\pm$ 0.4), $\Delta$-0.1 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9365, 0.9534, 0.9627} 44.9 ($\pm$ 0.5), $\Delta$-0.9 \\ % NTU activity classification

\textsc{w/o DanceDB} & %
    \cellcolor[rgb]{0.9709, 0.9579, 0.9502} 61.3 ($\pm$ 0.6), $\Delta$-0.7 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9248, 0.9479, 0.9606} 51.2 ($\pm$ 0.8), $\Delta$+1.5 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9131, 0.9423, 0.9584} 54.0 ($\pm$ 1.7), $\Delta$+1.9 &  % NTU motion prediction
    \cellcolor[rgb]{0.8956, 0.9340, 0.9552} 24.5 ($\pm$ 0.8), $\Delta$+1.1 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9599, 0.9645, 0.9670} 45.5 ($\pm$ 1.4), $\Delta$-0.3 \\ % NTU activity classification

\textsc{w/o NTU-60 \& 120} & %
    \cellcolor[rgb]{0.9131, 0.9423, 0.9584} 64.2 ($\pm$ 0.3), $\Delta$+2.2 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9306, 0.9506, 0.9616} 50.9 ($\pm$ 0.6), $\Delta$+1.2 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.8897, 0.9313, 0.9541} 54.9 ($\pm$ 0.5), $\Delta$+2.8 &  % NTU motion prediction
    \cellcolor[rgb]{0.8839, 0.9285, 0.9530} 24.7 ($\pm$ 0.5), $\Delta$+1.3 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.7809, 0.8784, 0.9301} 40.5 ($\pm$ 0.2), \textbf{$\Delta$-5.3} \\ % NTU activity classification

\textsc{NTU-60 Only} & %
    \cellcolor[rgb]{0.9599, 0.9645, 0.9670} 62.4 ($\pm$ 0.7), $\Delta$+0.4 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.8605, 0.9174, 0.9487} 53.2 ($\pm$ 0.6), $\Delta$+3.5 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9365, 0.9534, 0.9627} 53.3 ($\pm$ 0.3), $\Delta$+1.2 &  % NTU motion prediction
    \cellcolor[rgb]{0.7518, 0.8636, 0.9218} 26.4 ($\pm$ 0.9), \textbf{$\Delta$+3.0} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.7130, 0.8439, 0.9107} 39.2 ($\pm$ 0.2), \textbf{$\Delta$-6.6} \\ % NTU activity classification



\separator{Augmentations}
\textsc{w/o Axis Mirroring} & %
    \cellcolor[rgb]{0.9774, 0.9277, 0.8985} 59.8 ($\pm$ 1.2), $\Delta$-2.2 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9755, 0.9363, 0.9133} 48.2 ($\pm$ 1.0), $\Delta$-1.5 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9709, 0.9579, 0.9502} 51.5 ($\pm$ 0.9), $\Delta$-0.6 &  % NTU motion prediction
    \cellcolor[rgb]{0.9737, 0.9449, 0.9280} 22.9 ($\pm$ 0.4), $\Delta$-0.5 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9248, 0.9479, 0.9606} 44.5 ($\pm$ 0.5), $\Delta$-1.3 \\ % NTU activity classification

\textsc{w/o Random Scaling} & %
    \cellcolor[rgb]{0.9599, 0.9645, 0.9670} 62.3 ($\pm$ 0.5), $\Delta$+0.3 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9073, 0.9396, 0.9573} 51.8 ($\pm$ 0.5), $\Delta$+2.1 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9190, 0.9451, 0.9595} 53.8 ($\pm$ 0.2), $\Delta$+1.7 &  % NTU motion prediction
    \cellcolor[rgb]{0.6937, 0.8341, 0.9052} 26.9 ($\pm$ 0.3), \textbf{$\Delta$+3.5} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.5665, 0.7687, 0.8685} 36.5 ($\pm$ 0.5), \textbf{$\Delta$-9.3} \\ % NTU activity classification

\textsc{w/o Joint Jitter} & %
    \cellcolor[rgb]{0.9657, 0.9672, 0.9681} 62.1 ($\pm$ 1.1), $\Delta$+0.1 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9190, 0.9451, 0.9595} 51.4 ($\pm$ 0.7), $\Delta$+1.7 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 52.9 ($\pm$ 1.1), $\Delta$+0.8 &  % NTU motion prediction
    \cellcolor[rgb]{0.9248, 0.9479, 0.9606} 24.1 ($\pm$ 0.9), $\Delta$+0.7 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.8897, 0.9313, 0.9541} 43.4 ($\pm$ 0.9), $\Delta$-2.4 \\ % NTU activity classification

\textsc{w/o Slow Down} & %
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 61.9 ($\pm$ 0.4), $\Delta$-0.1 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9131, 0.9423, 0.9584} 51.5 ($\pm$ 1.3), $\Delta$+1.8 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9365, 0.9534, 0.9627} 53.3 ($\pm$ 0.5), $\Delta$+1.2 &  % NTU motion prediction
    \cellcolor[rgb]{0.8255, 0.9008, 0.9423} 25.6 ($\pm$ 1.5), \textbf{$\Delta$+2.2} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.8897, 0.9313, 0.9541} 43.3 ($\pm$ 0.6), $\Delta$-2.5 \\ % NTU activity classification

\textsc{w/o Speed Up} & %
    \cellcolor[rgb]{0.9728, 0.9493, 0.9354} 60.9 ($\pm$ 0.5), $\Delta$-1.1 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9540, 0.9617, 0.9659} 50.2 ($\pm$ 0.6), $\Delta$+0.5 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9657, 0.9672, 0.9681} 52.2 ($\pm$ 0.4), $\Delta$+0.1 &  % NTU motion prediction
    \cellcolor[rgb]{0.9599, 0.9645, 0.9670} 23.5 ($\pm$ 0.7), $\Delta$+0.1 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9131, 0.9423, 0.9584} 44.1 ($\pm$ 1.5), $\Delta$-1.7 \\ % NTU activity classification

\textsc{w/o Frame Dropout} & %
    \cellcolor[rgb]{0.9737, 0.9449, 0.9280} 60.6 ($\pm$ 0.6), $\Delta$-1.4 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 49.6 ($\pm$ 0.6), $\Delta$-0.1 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9691, 0.9665, 0.9649} 51.9 ($\pm$ 1.4), $\Delta$-0.2 &  % NTU motion prediction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 23.7 ($\pm$ 0.8), $\Delta$+0.3 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9365, 0.9534, 0.9627} 44.9 ($\pm$ 0.7), $\Delta$-0.9 \\ % NTU activity classification

\textsc{w/o Joint Dropout} & %
    \cellcolor[rgb]{0.7905, 0.8833, 0.9329} 68.8 ($\pm$ 1.4), \textbf{$\Delta$+6.8} &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.7130, 0.8439, 0.9107} 56.7 ($\pm$ 2.6), \textbf{$\Delta$+7.0} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9700, 0.9622, 0.9576} 51.8 ($\pm$ 1.1), $\Delta$-0.3 &  % NTU motion prediction
    \cellcolor[rgb]{0.8488, 0.9119, 0.9466} 25.3 ($\pm$ 0.8), \textbf{$\Delta$+1.9} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.8488, 0.9119, 0.9466} 42.1 ($\pm$ 0.9), \textbf{$\Delta$-3.7} \\ % NTU activity classification

\textsc{w/ Random Rotation} & %
    \cellcolor[rgb]{0.9423, 0.9562, 0.9638} 63.2 ($\pm$ 0.6), $\Delta$+1.2 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.8780, 0.9257, 0.9519} 52.7 ($\pm$ 1.2), $\Delta$+3.0 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9190, 0.9451, 0.9595} 53.9 ($\pm$ 0.8), $\Delta$+1.8 &  % NTU motion prediction
    \cellcolor[rgb]{0.8722, 0.9230, 0.9509} 24.9 ($\pm$ 0.7), $\Delta$+1.5 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.9802, 0.9148, 0.8764} 48.1 ($\pm$ 0.3), $\Delta$+2.3 \\ % NTU activity classification

\textsc{Spatial Only} & %
    \cellcolor[rgb]{0.9540, 0.9617, 0.9659} 62.5 ($\pm$ 0.9), $\Delta$+0.5 &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.9131, 0.9423, 0.9584} 51.5 ($\pm$ 1.7), $\Delta$+1.8 &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9073, 0.9396, 0.9573} 54.2 ($\pm$ 2.0), $\Delta$+2.1 &  % NTU motion prediction
    \cellcolor[rgb]{0.8547, 0.9146, 0.9476} 25.2 ($\pm$ 0.8), $\Delta$+1.8 &  % HDM05 motion prediction
    \cellcolor[rgb]{0.8430, 0.9091, 0.9455} 42.0 ($\pm$ 0.9), \textbf{$\Delta$-3.8} \\ % NTU activity classification

\textsc{Temporal Only} & %
    \cellcolor[rgb]{0.6840, 0.8291, 0.9024} 71.6 ($\pm$ 0.2), \textbf{$\Delta$+9.6} &  % NTU skeleton reconstruction
    \cellcolor[rgb]{0.6161, 0.7947, 0.8830} 58.8 ($\pm$ 3.4), \textbf{$\Delta$+9.1} &  % HMD05 skeleton reconstruction
    \cellcolor[rgb]{0.9482, 0.9589, 0.9649} 52.8 ($\pm$ 0.3), $\Delta$+0.7 &  % NTU motion prediction
    \cellcolor[rgb]{0.5300, 0.7456, 0.8561} 28.4 ($\pm$ 2.0), \textbf{$\Delta$+5.0} &  % HDM05 motion prediction
    \cellcolor[rgb]{0.0196, 0.1882, 0.3804}\color{white} 23.0 ($\pm$ 0.1), \textbf{$\Delta$-22.8} \\ % NTU activity classification



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bottomrule 
\end{tabular}
\end{scriptsize}
\vspace{-1mm}
\end{table}

==> Skeleton Embeddings – NeurIPS SSL Workshop 2022/tables/dataset_statistics.tex <==
\begin{table}[t]
\centering
\small
\caption{Datasets used in this work. Training set of datasets marked with $\ast$ are used to pre-train skeleton representation with SimCLR, those marked with $\diamond$ are used for downstream task training.}
\label{table:dataset_statitics}
\begin{scriptsize}
\begin{tabular}{%
    m{0.25\columnwidth}
    >{\raggedleft\arraybackslash}m{0.13\columnwidth}
    >{\raggedleft\arraybackslash}m{0.12\columnwidth}
    >{\raggedleft\arraybackslash}m{0.09\columnwidth}
    >{\centering\arraybackslash}m{0.11\columnwidth}
    >{\centering\arraybackslash}m{0.13\columnwidth}
}
\toprule

\textbf{\textsc{Dataset}} & %
\textbf{\textsc{Number of Train~Frames}} & %
\textbf{\textsc{Number of Test~Frames}} & %
\textbf{\textsc{Unique Human Subjects}} & %
\textbf{\textsc{Frames per Second}} & %
\textbf{\textsc{Recording Device}} \\
\midrule

\textsc{NTU RGB+D 60}$^{\ast\diamond}$~\cite{shahroudy2016ntu} & %
    3,328,560 (8\%) &       % number of train frames
    1,456,493 (92\%) &      % number of test frames
    40 (22\%)  &            % number of subjects
    30  &                   % framerate
    Depth Camera \\     % device
    
\textsc{NTU RGB+D 120}$^\ast$~\cite{liu2020ntu} & 
    4,324,668 (11\%) &      % number of train frames
    -- &                    % number of test frames
    66 (37\%) &             % number of subjects
    30 &                    % framerate
    Depth Camera \\     % device

\textsc{Trinity Speech-Gesture}$^\ast$~\cite{trinity} & 
    4,579,806  (11\%) &     % number of train frames
    -- &                    % number of test frames
    1 (1\%) &               % number of subjects
    120 &                   % framerate
    MoCap System \\             % device

\textsc{Talking with Hands}$^\ast$~\cite{talkingwithhands} & 
    25,680,106 (64\%) &     % number of train frames
    -- &                    % number of test frames
    50 (28\%) &             % number of subjects
    90 &                    % framerate
    MoCap System \\            % device

\textsc{DanceDB}$^\ast$~\cite{dancedb} & 
    1,679,209 (4\%) &       % number of train frames
    -- &                    % number of test frames
    17 (9\%) &              % number of subjects
    120 &                   % framerate
    MoCap System \\            % device

\textsc{HDM05}$^\diamond$~\cite{cg-2007-2}  & 
    492,340 (1\%) &                    % number of train frames
    123,085 (8\%) &        % number of test frames
    5 (3\%) &               % number of subjects
    120 &                   % framerate
    MoCap System \\             % device

\midrule
\textsc{Total} & 40,084,689 & 1,579,578 & 179  & -- \\
\bottomrule
\end{tabular}
\end{scriptsize}
\vspace{-1mm}
\end{table}







==> Skeleton Embeddings – NeurIPS SSL Workshop 2022/tables/hyper_parameter_training.tex <==
\begin{table}[t!]
\centering
\caption{Hyper-parameter used in pretraining and downstream tasks}
\begin{scriptsize}
\normalsize
\begin{tabular}{%
      >{\centering\arraybackslash}m{3.5cm}%
      >{\centering\arraybackslash}m{3.5cm}%
      >{\centering\arraybackslash}m{3.5cm}%
}


\toprule
& Pretraining & Downstream Task\\
\midrule
Batch Size              & 8096           & 1024  \\
Training Epochs         & 500            & 200   \\
Optimizer               & Lars Momentum  & Adam  \\
Learning Rate           & 0.01           & 0.01  \\
LR Warmup               & 10             & -     \\
LR Update Schedule      & cosine         & -     \\
Backbone Feature Size   & 128   & -              \\
Head Latent Size        & 256   & -              \\
Head Output Size        & 128   & -              \\
Head Output Size        & 128   & -              \\

\bottomrule
\end{tabular}
\end{scriptsize}
\end{table}


\begin{table}[t!]
\centering
\caption{Network Parameter used in pretraining and downstream tasks}
\begin{scriptsize}
\normalsize
\begin{tabular}{%
      >{\centering\arraybackslash}m{5cm}%
      >{\centering\arraybackslash}m{3.5cm}%
}
\toprule
& Trainable Parameters                          \\
\midrule
SimCLR &                                        \\
Encoder (ST-GCN)             & 0.968458M        \\
Encoder (MLP)                & 1.351168M        \\[0.1cm]
Frozen &                                        \\
Activity Classification         & 0.00774M      \\
Motion Prediction Frozen        & 2.905182M     \\
Skeleton Reconstruction Frozen  & 2.905182M     \\[0.1cm]
Fine-Tune &                                     \\
Activity Classification         & 0.843206M     \\
Motion Prediction Frozen        & 3.740648M     \\
Skeleton Reconstruction Frozen  & 3.740648M     \\
\bottomrule
\end{tabular}
\end{scriptsize}
\vspace{10cm}
\end{table}




==> Skeleton Embeddings – NeurIPS SSL Workshop 2022/tables/hyper_parameters.tex <==
\begin{table}[h]
\centering
\caption{Augmentations hyper-parameters for pre-training with probabilities and strengths}
\label{table:hyperparameters}
\begin{scriptsize}
\normalsize
\begin{tabular}{%
       >{\centering\arraybackslash}m{2.5cm}%
       >{\centering\arraybackslash}m{2.5cm}%
       >{\centering\arraybackslash}m{2.5cm}%
}
\toprule

Augmentation    &  Probability  &  Strength                     \\

\midrule

Axis mirroring  &  0.5          &  -                            \\ 
Random Scale    &  0.7          &  $\mu$: 0, $\sigma^2$: 0.02   \\
Joint Jitter    &  0.5          &  $\mu$: 0, $\sigma^2$: 0.02   \\
Slow down       &  0.5          &  0.5x-0.9x                    \\ 
Speed up        &  0.5          &  1.2-2x                       \\ 
Frame Dropout   &  0.5          &  0.5                          \\ 
Joint Dropout   &  0.5          &  0.5                          \\ 
Random rotation &  0.6          &  $\pm \pi$                    \\

\bottomrule
\end{tabular}
\end{scriptsize}
\end{table}


